Differentially Private Histograms under Continual Observation: Streaming Selection into the Unknown

We generalize the continuous observation privacy setting from Dwork et al. '10 and Chan et al. '11 by allowing each event in a stream to be a subset of some (possibly unknown) universe of items. We design differentially private (DP) algorithms for histograms in several settings, including top-$k$ selection, with privacy loss that scales with polylog$(T)$, where $T$ is the maximum length of the input stream. We present a meta-algorithm that can use existing one-shot top-$k$ DP algorithms as a subroutine to continuously release private histograms from a stream. Further, we present more practical DP algorithms for two settings: 1) continuously releasing the top-$k$ counts from a histogram over a known domain when an event can consist of an arbitrary number of items, and 2) continuously releasing histograms over an unknown domain when an event has a limited number of items.

==> binaryMechanism.tex <==
%!TEX root = main.tex
\section{Binary Mechanism} % (fold)

We first discuss the classical Binary Mechanism from \citet{ChanShSo11} that provides a running count for a stream of bits.  Due to recent work comparing the overall privacy loss for Laplace noise and Gaussian noise from \cite{CesarRo20} and \cite{CanonneKaSt20}, we will use Gaussian noise, rather than Laplace noise in the original algorithm.  We first need to set up some notation.  We will write $b_j(t) \in \{ 0,1\}$ to be the $j$th digit in the binary representation of $t$, i.e. $t = \sum_{j = 0}^{\lfloor \log_2(t) \rfloor} b_j(t) 2^j$.  

We then present the Binary Mechanism in Algorithm~\ref{algo:BinaryMechanism}
\begin{algorithm}[h!]
	\caption{$\BinMech$; Return a running count on a single stream}
	\begin{algorithmic}
		\State \textbf{Input:} Stream $\omega_{1:T} = \omega_1, \cdots, \omega_T$, where $\omega_t\in \{ 0,1\}$ for all $t \in [T]$.
		\State \textbf{Output:} Noisy counts $\hat{y}_{1:T} = \hat{y}_1, \cdots, \hat{y}_T$.
		\State Initialize: $\bbr$ is a table of zeros of size $\lfloor \log_2(T) \rfloor+ 1$ by $T$.
		\For{$t = 1, \cdots, T$}
			\State Write $t = \sum_{j = 0}^{\lfloor \log_2(t)\rfloor}b_j(t) 2^j$
			\State $ i \gets \min\{j:b_j(t) \neq 0 \} $
			\For{$j= 0, \cdots,i $}
				\State $\bbr(j,t/2^j) \gets \sum_{\ell = t/2^j}^t \omega_\ell $
				\State $\hat\bbr(j,t/2^j) \gets \bbr(j,t/2^j) + \Normal{0}{(\log_2(T)+ 1)  \cdot \sigma^2}$
			\EndFor
			$\hat{y}_t \gets \sum_{j = 0}^{\lfloor \log_2(t) \rfloor} b_j(t) \hat\bbr(j,t/2^j)$
		\EndFor
		\State Return $\hat{y}_{1:T} = \hat{y}_1, \cdots, \hat{y}_T$.	
	\end{algorithmic}\label{algo:BinaryMechanism}
\end{algorithm}

We now state the privacy guarantee in terms of zCDP.
\begin{lemma}
The $\BinMech(\omega_{1:T})$ is $\tfrac{1}{2\sigma^2}$-zCDP and hence $\left(\tfrac{1}{2\sigma^2}+ \tfrac{1}{\sigma}\sqrt{\tfrac{1}{2}\ln(1/\delta')},\delta'\right)$-DP for all $\delta'> 0$.
\end{lemma}
\begin{proof}
The proof follows the same argument as in \cite{ChanShSo11}.  Rather than outputting the noisy counts, we instead consider outputting the entire table of partial counts $\{ \hat\bbr(j,\ell) : j \in [ \lfloor\log_2(T)\rfloor + 1], \ell \in [T] \}$.   Let $\omega_{1:T}$ and $\omega'_{1:T}$ be two neighboring streams with partial sum tables $\bbr$ and $\bbr'$, respectively.  Due to the way we defined neighbors, these two partial sum counts can differ in at most $\log_2(T) + 1$ cells and can differ in each cell by at most 1.  Hence, the $\ell_2$-sensitivity of the partial sum table is at most $\log_2(T) + 1$, and by adding $\Normal{0}{(\lfloor \log_2(T) \rfloor + 1) \sigma^2}$ to each cell's true count ensures $\frac{1}{2\sigma^2}$-zCDP.  
\end{proof}

==> knownDomain.tex <==
%!TEX root = main.tex
\section{Known Domain with Bounded User Contribution} % (fold)


